Automated Characterization of Software Vulnerabilities

Preventing vulnerability exploits is a critical software maintenance task, and software engineers often rely on Common Vulnerability and Exposure (CVEs) reports for information about vulnerable systems and libraries. These reports include descriptions, disclosure sources, and manually-populated vulnerability characteristics such as root cause from the NIST Vulnerability Description Ontology (VDO). This information needs to be complete and accurate so stakeholders of affected products can prevent and react to exploits of the reported vulnerabilities. However, characterizing each report requires significant time and expertise which can lead to inaccurate or incomplete reports. This directly impacts stakeholders ability to quickly and correctly maintain their affected systems. In this study, we demonstrate that VDO characteristics can be automatically detected from the textual descriptions included in CVE reports. We evaluated the performance of 6 classification algorithms with a dataset of 365 vulnerability descriptions, each mapped to 1 of 19 characteristics from the VDO. This work demonstrates that it is feasible to train classification techniques to accurately characterize vulnerabilities from their descriptions. All 6 classifiers evaluated produced accurate results, and the Support Vector Machine classifier was the best-performing individual classifier. Automating the vulnerability characterization process is a step towards ensuring stakeholders have the necessary data to effectively maintain their systems.

==> aboutClassifiers.tex <==
\section{Classifiers}
\label{sec:aboutClassifiers}
We compared the performance of \numClassifiers{} classification algorithms for this task, using implementations of each algorithm provided by the Weka data mining tool~\cite{hall2009weka}. 3 of the classifiers are individual, and 3 are ensemble learners, which merge results from multiple classifiers in different ways. Here, we explain each algorithm, selected based on suitability for the given task: 
%\danielle{My goal with these descriptions was to make them  approachable for people not in the ML domain. I reviewed the proceedings from the 3 instances of this conference, and there was only 1 paper that used ML: https://ieeexplore.ieee.org/document/8077800. It's actually kind of similar, they used 7 classifiers to predict if a SDL activities were required for a SW project. Anyway, with this intended audience in mind I did not include formulas.}


%\hl{It looks to me that V.A and V.B can be mentioned here. Then after that you can describe each algorithm. Then the paper reads as, you present an approach (i.e. using supervised learning, then you mention the data used for training and the process for preparing the data, after that you mention the algorithms to be used. I haven't read the paper throughly, just think about this and see if this is a better structure. Make the call.}

\subsection{Na\"{i}ve Bayes}
This classifier uses the labeled training data to apply Bayes' theorem~\cite{bayes1763lii} of \textit{posterior probability} to classify test data ~\cite{naivebayes}. During the training phase, the algorithm keeps track of two things: the number of \textit{documents} (vulnerability descriptions) assigned to each class, and the number of times each \textit{word} was assigned to each class. For a new test input, the probability that the document belongs to a class is the product of the \textit{total probability of the class} and the probability that the document belongs in the class based on its words. The input is then assigned to the class with the highest probability.

\subsection{Decision Tree}
These classifiers recursively divide data using a specific \textit{condition}. For text classification, the condition is the presence or absence of a word(s) in each document (vulnerability description) A classification tree iteratively splits the data based on the presence or absence of 1 word. This is known as a \textit{single attribute split}, where the selected word provides \textit{maximum distance} between classes~\cite{aggarwal2012survey}.  The Weka tool implements a C4.5 decision tree~\cite{Quinlan1993}, which selects the word with the highest \textit{normalized information gain}~\cite{quinlan1986induction}. 

\subsection{Support Vector Machine}
These linear classifiers, known as SVMs, finds the best \textit{separating hyper-plane} to distinguish classes of data by identifying the \textit{maximum margin of separation} between the outermost points (on the plane) for each class~\cite{aggarwal2012survey,svm} using a linear discriminant function. The Weka implementation used in this study applies Sequential Minimizing Optimization~\cite{smoForsvm,Keerthi2001} to find the best separating hyper-plane, and \textit{pairwise} classification to handle more than 2 classes~\cite{Hastie1998}.

\subsection{Random Forest}
This algorithm is an \textit{ensemble learner} that builds multiple \textit{random} trees and merges the results with the goal of increased accuracy~\cite{randomforest}. This classifier builds \textit{random trees}, which are decision trees that use a \textit{random} approach instead of a rule-based approach. The input data is randomly split between the trees and each tree considers only a random subset of features (words) for each input (vulnerability description). Then, each tree selects a class using the condition-based approach described above. The results are merged by using a majority-voting scheme and the class output by the most trees is selected.

\subsection{AdaBoost-SVM}
AdaBoost, or Adaptive Boosting, is another \textit{ensemble learner} which applies a technique called \textit{boosting}. This is a type of \textit{voting} mechanism where the results from multiple instances of a classifier are merged with the goal of producing higher accuracy results. The algorithm iteratively trains, and it updates a weight for each item in the dataset based on how successfully it was classified in the previous iteration. The Weka implementation used in this study~\cite{Freund1996} calculates weight for each item as a logarithmic function of its error. We ran preliminary experiments to select a base classifier for this ensemble, and SVM had the best results. 

\subsection{Majority Vote}
This \textit{ensemble learner} can merge the results of multiple \textit{different} classification algorithms. Each classifier is trained individually, and for each item in the test set, the class selected by the \textit{majority} of classifiers is assigned~\cite{Kuncheva2004,Kittler1998}. In our experiment we executed this classifier using 1 of each of the previous 5 algorithms: AdaBoost, SVM, Random Forest, Decision Tree, and Na\"{i}ive Bayes.

\subsection{Hyper-Parameter Optimization}
\label{sec:optimize}
Classification algorithms have many configurable parameters, but most implementations provide a set of default values for them based on recommendations from literature. However, each algorithm typically has a subset of \textit{hyper-parameters} that must be \textit{optimized} to get the best performance for a given dataset. As an example, a Support Vector Machine can use a number of different \textit{kernel functions} for separating hyper-planes. For each of the \numClassifiers{} classifiers, we performed a series of 10-fold cross validation experiments to tune the hyper-parameters for our dataset. We provide the full Weka ``schemes" (configurations) for each classifier in Table~\ref{tab:wekaSchemes} for replication purposes. These schemes can be input into Weka to perform a classification using our exact configurations. Note that Na\"{i}ve Bayes did not have any parameters.

\begin{table*}
\centering
\caption{Classification Algorithm Hyper-Parameter Configuration Schemes Used in Weka Tool}
\begin{tabular}{|l|p{15.5cm}|}
\hline
\textbf{Classifier} & \textbf{Weka Schema}                                                                                                     \\ \hline
Random Forest       & weka.classifiers.trees.RandomForest,-P 100 -O -I 320 -num-slots 1 -K 1 -M 1.0 -V 0.001 -S 123 -B                                                                                                                                                                                                             \\ \hline
Decision Tree       & weka.classifiers.trees.J48 -C 0.4 -M 0                                                                                              \\ \hline
SVM                 & weka.classifiers.functions.SMO -C 0.5 -L 0.001 -P 1.0E-12 -N 0 -V 10 -W 123 -K "weka.classifiers.functions.supportVector.PolyKernel -E 1.0 -C 250007" -calibrator "weka.classifiers.functions.Logistic -R 1.0E-8 -M -1 -num-decimal-places 4"                                                                                                                                             \\ \hline
AdaBoost            & weka.classifiers.meta.AdaBoostM1,-P 100 -S 123 -I 100 -W weka.classifiers.functions.SMO -- -C 0.5 -L 0.001 -P,1.0E-12 -N 0 -V 10 -W 123 -K,"weka.classifiers.functions.supportVector.PolyKernel -E 1.0 -C,250007" -calibrator "weka.classifiers.functions.Logistic -R 1.0E-8,-M -1 -num-decimal-places 4"                                                                                       \\ \hline
MajorityVote        & weka.classifiers.meta.Vote,-S 123 -B "weka.classifiers.bayes.NaiveBayes " -B,"weka.classifiers.functions.SMO -C 0.5 -L 0.001 -P 1.0E-12 -N 0 -V 10 -W,123 -K \textbackslash{}"weka.classifiers.functions.supportVector.PolyKernel -E 1.0 -C,250007\textbackslash{}" -calibrator \textbackslash{}"weka.classifiers.functions.Logistic -R,1.0E-8 -M -1 -num-decimal-places 4\textbackslash{}"" -B,"weka.classifiers.trees.J48 -C 0.4 -M 0" -B,"weka.classifiers.trees.RandomForest -P 100 -O -I 320 -num-slots 1 -K 1,-M 1.0 -V 0.001 -S 123" -B "weka.classifiers.meta.AdaBoostM1 -P 100,-S 123 -I 100 -W weka.classifiers.functions.SMO -- -C 0.5 -L 0.001 -P 1.0E-12,-N 0 -V -1 -W 123 -K,\textbackslash{}"weka.classifiers.functions.supportVector.PolyKernel -E 1.0 -C,250007\textbackslash{}" -calibrator \textbackslash{}"weka.classifiers.functions.Logistic -R,1.0E-8 -M -1 -num-decimal-places 4\textbackslash{}"" -R MAJ \\ \hline
\end{tabular}
\label{tab:wekaSchemes}
\end{table*}

==> aboutMetrics.tex <==
\section{Evaluation Metrics for Classifiers}
\label{sec:aboutMetrics}
We used 6 evaluation metrics for classification~\cite{sokolova2009systematic} to compare the performance of each algorithm for the task of assigning 1 of the \numAttributes{} vulnerability characterization attributes to each of the \numCVEs{} vulnerability descriptions. During an evaluation, the true class for items in the training set are known. Therefore, the performance measures are calculated using comparisons of the \textit{predicted vs true conditions}, often represented as a confusion matrix as shown in Figure~\ref{fig:confusionExample}. A \textit{true positive} is an item \textul{correctly assigned} to a class, while a \textit{false positive} is an item \textul{incorrectly assigned} to a class. Likewise a \textit{true negative} is an item \textul{correctly not assigned} to a class, and a \textit{false negative} is an item \textul{incorrectly not assigned} to a class. 

Once the classifier finishes assigning data to classes, the predicted class for each item in the data set is then compared to its true class. Then, the sums of the 4 values (eg. total \# of true positives) are calculated for each class.
\begin{figure}[ht]
\centering
\includegraphics[width=120px,height=100px]{Figs/Confusionmatrix.png}
\caption{Confusion Matrix for Evaluating Classifiers~\cite{raschka2014overview}}
\label{fig:confusionExample}
\end{figure}

The following metrics use these ``total" values to measure specific abilities of a classification algorithm. Calculating each is important for having a balanced perspective on the algorithm's performance. For each classifier in our study, these values were calculated for all \numAttributes{} classes. The methodology for establishing the training data and conducting the experiments are explained in Section~\ref{sec:method} and the results are reported in Section~\ref{sec:results}. 

\subsection{Precision}
The ratio of the number of items \textit{correctly} assigned to a class to the \textit{total number} of items assigned to a class~\cite{olson2008advanced}. To calculate a classifier's precision $P$ for an individual class, $P = \frac{TP}{TP + FP}$ where $TP$ is the number of true positives (correct assignments) and $FP$ is the number of false positives (items incorrectly assigned to the class). When $P=1$, this means that \textit{every} item in the class was correctly assigned. As an example, the precision of a search engine is a measure of how many results returned for a search were relevant to the query. In our work, this value measured how often a classifier assigned a vulnerability description to the correct characterization. 

\subsection{Recall} The ratio of the number of items \textit{correctly} assigned to a class to the \textit{total number} of items that actually belong to the class~\cite{olson2008advanced}. This is calculated for an individual class as $R = \frac{TP}{TP + FN}$, where $FN$ is the number of false negatives (items incorrectly not assigned to the class). When $R = 1$, this means that the classifier correctly assigned \textit{every} item that should have been assigned to the class. As an example, the recall of a search engine is a measure of how many existing relevant results in the search space were returned. In our work, this value measured how often a classifier correctly identified all the vulnerability descriptions that should be assigned to each characterization.

\subsection{Accuracy} This is a classic baseline metric for evaluating the overall performance of a classifier~\cite{olson2008advanced}. Simply put, it is the percentage of correctly classified data across all classes. It is calculated for a classifier as $A = \frac{TP + TN}{TP + FP + TN +FN}$.

\subsection{Kappa Statistic} This is another baseline metric for evaluating a classifier's overall performance. It is a measurement of pairwise \textit{agreement} between two ratings of the same item~\cite{Carletta:1996:AAC:230386.230390}. In the context of classification, it measures whether a classifier (`rating 1') performed better at assigning items to a class than \textit{random} assignment (`rating 2'). This metric is calculated using the ``success rate" of a classifier ($SR_{C}$) and of a random assignment ($SR_{R}$), which is the total number of \textit{true positives} ($TP$) for all classes, or $SR = \sum_{n=1}^{\text{\# classes}}TP_{n}$. Kappa is therefore $K = \frac{SR_{C}}{1-SR_{R}}$. When $K=1$, the classifier had perfect accuracy, but a value of 0 means the classifier performed the same as random assignment.

\subsection{F-Measure} Also known as F1 score or F-score, it is the \textit{harmonic mean} of the precision and recall~\cite{van1979information}. We calculate this metric alongside accuracy because it gives equal importance to both precision and recall. In our context, its equally important to identify all applicable vulnerability descriptions for a characterization AND characterize every vulnerability description correctly. It is calculated for an individual class as $F = 2 * \frac{P * R}{P + R}$, where $P$ is the precision and $R$ is the recall. When $F = 1$ for an individual class, all of the items assigned to that class belonged there, and it assigned all the appropriate items in the dataset. In our work, we use this metric to measure each classifiers overall performance across classes and to compute the ratio of best performance.

\subsection{Ratio of Best Performance}We introduce this metric as a combined way of summarizing a classifiers performance for each individual characterization while also comparing all of the algorithms evaluated. For an individual algorithm, it indicates the ratio of classes it had the \textit{best} performance for among all algorithms evaluated, to the total number of classes. For each of the \numAttributes{} characterization classes in our study, we marked the algorithm with the best F-measure value with a `1' and the others with a `0'. In the case of a tie, each algorithm was assigned a `1'. Then, the \textit{ratio of best performance} was calculated for each classifier as $RBP = \frac{\text{\# of 1s}}{\text{total \# of classes}}$, where `number of 1s' indicates the number of classes where the algorithm was the best performer.


==> aboutVDO.tex <==
\section{Background and Definitions}
\label{sec:aboutVDO}

\subsection{Vulnerability Reports (CVEs)}

The Computer Security Division of the National Institute of Standards and Technology (NIST) in the United States maintains an online repository of CVE reports called the National Vulnerability Database (NVD)~\cite{booth2013national}. Figure~\ref{fig:sampleCVE} is a CVE report from the NVD website featuring \circled{1} a unique ID, \circled{2} a free-text description of the vulnerability, \circled{3} standardized CVSS severity scores~\cite{4042667}, \circled{4} disclosures \& sources, and \circled{5} standardized Common Weakness Enumerations (CWEs)~\cite{enumeration2017community} representing the root cause. 
\begin{figure}
\centering
\includegraphics[width=\linewidth,height=300px]{Figs/CVEExampleLong.png}
\caption{Example of a Vulnerability Report from the NVD}
\label{fig:sampleCVE}
\end{figure}

\subsection{Vulnerability Characterizations} 
The stated purpose of the NIST Vulnerability Description Ontology (VDO) is to establish a \textit{``common vocabulary"} which would standardize the vulnerability management process and ``enable automated tools to assist in the analysis process"\cite{booth2016draft}. This motivates our aim to alleviate the problems associated with manual report generation and develop a solution which uses the descriptive text in each report to accurately and \textit{automatically} identify the relevant characterization from the ontology.

The VDO is a framework consisting of \textit{vulnerability characterizations} organized into 18 higher level categories (eg. \textit{Mitigation}, \textit{Scope}). Categories have cardinal relationships with each other to represent the supplemental information characterizations provide to each other (eg. a \textit{Logical Impact} may be associated with only one \textit{Scope}). Further, each category is assigned a \textit{usage}, such that assigning a characterization from that category to a vulnerability is either \textit{mandatory, recommended, or optional}. Figure~\ref{fig:vdoDiagram} visualizes the existing categories in the NIST ontology, their characterization attributes, and the relationships between them. This figure was constructed from the specifications in the ontology report~\cite{booth2016draft}.  


\begin{figure*}
\centering
\includegraphics[width=\linewidth]{Figs/VDO_Figure.png}
\centering\caption{The NIST Vulnerability Description Ontology (VDO)}
\label{fig:vdoDiagram}
\end{figure*}

\subsection{Vulnerability Characteristics Selected for this Study}\label{sec:attributes}
To evaluate the \textit{feasibility} of the proposed classification approach, we selected a subset of \numAttributes{} characterizations from \numGroups{} of the VDO's categories. For our evaluation, we included \numAttributes{} characterizations that we were able to manually identify relevant CVEs for (see Section~\ref{sec:trainingData}). 
In this section, we define each selected characterization and the ontology categories they come from. Definitions are derived from the VDO report~\cite{booth2016draft} unless otherwise noted. VDO descriptions for each characterization are also provided in Table~\ref{tab:attributeDescriptions}. 

\noindent\textbf{Mitigation}: (Optional) A software system may have \textit{built-in exploit prevention} such that if a vulnerability exists, it is not able to be exploited as intended. Typically, these are designed into the system to be part of its intended use. 

\noindent{The following mitigations were included in our study:}
\begin{itemize}
\item{} \textbf{Address Space Layout Randomization (ASLR)}~\cite{team2003pax}: Random arrangement of address spaces for data, used to prevent exploits of memory corruption vulnerabilities.
\item{} \textbf{Multi-Factor Authentication}~\cite{owen2008multi}: The requirement that more than 1 piece of `evidence' be provided before access is granted. Evidence typically includes 2 or more of something \textit{known} (eg. password), something \textit{possessed} (eg. RSA token), or something you \textit{are} (eg. fingerprint).
\item{} \textbf{Sandboxed}~\cite{Goldberg:1996:SEU:1267569.1267570}: Software components have been sandboxed when they are separated into protected environments.
\item{} \textbf{HTTP Public Key Pinning (HPKP)}~\cite{evans2015public}: Use of a set of public keys only delivered to the client, trusted only for that clients domain name to prevent impersonation.
\item{} \textbf{HTTP Strict Transport Security (HSTS)}~\cite{hodges2012http}: Web server only allows browsers to connect to it using HTTPS, used to prevent cookie hijacking.
\item{} \textbf{Physical Security}: A physical entity used to prevent attack or exploit (eg. security camera).
\end{itemize}

\noindent\textbf{Impact Method}: (Mandatory) How a vulnerability can be exploited. Each impact method in the VDO more specifically indicates \textit{what is exploited} in an attack.

\noindent{We included the following impact methods in our study:}
\begin{itemize}
\item{} \textbf{Context Escape}: The vulnerability permits an attacker to escape a sandboxed or otherwise protected environment by exploiting an unverified trust \textit{mechanism}.
\item{} \textbf{Trust Failure}: A trust \textit{relationship} that was not verified (eg. unsanitized input) was exploited.
\item{} \textbf{Man-in-the-Middle}~\cite{callegati2009man}: An attacker captures and potentially alters communication between two unaware parties, typically by exploiting an unverified trust \textit{mechanism}.
\end{itemize}


\noindent\textbf{Logical Impact}: (Mandatory) A successful exploit allows an attacker to receive some sort of information, or perform some action, that would not otherwise be permitted. These characterizations describe \textit{what the exploit allows} the attacker to do at the software level.

\noindent{We included the following logical impacts in our study:}
\begin{itemize}
\item{} \textbf{Write}: The attacker can modify or add data.
\item{} \textbf{Read}: The attacker has access to restricted data.
\item{} \textbf{Service Interrupt}: The attacker can affect the availability of the software.
\item{} \textbf{Indirect Disclosure}: A less extreme form of read access, where information is indirectly gained from another source (eg. traffic analysis).
\item{} \textbf{Privilege Escalation}: An attacker can perform actions which were not authorized. 
\end{itemize}

\noindent\textbf{Location}: (Optional) An indication of \textit{which part of the system is affected} by a successful exploit.

\noindent{We included the following locations in our study:}
\begin{itemize}
\item{} \textbf{Memory}: An exploit allows the logical impact to occur in memory.
\item{} \textbf{File System}: An exploit allows the logical impact to occur within the file system.
\item{} \textbf{Network Traffic}: An exploit allows the logical impact to occur in the network traffic of the application.
\end{itemize}


\noindent\textbf{Scope}: (Mandatory) A measurement of \textit{constraint a successful exploit has}, meaning how much of the system the attacker can access. An example from the VDO is that the `Read' logical impact gives the attacker unlimited access to the entire system.

\noindent{We included both scopes in our study:}
\begin{itemize}
\item{} \textbf{Limited}: A restriction exists which limits the impact an exploit has on the system (eg. may only occur in memory)
\item{} \textbf{Unlimited}: The impact of the exploit has no boundary and can affect the entire system.
\end{itemize}

\begin{table*}
\centering
\caption{Characterizations from NIST Vulnerability Description Ontology Used to Classify Vulnerabilities}
\begin{tabular}{|l|l|p{11.5cm}|}
\hline
\multicolumn{1}{|c|}{\textbf{Group}} & \multicolumn{1}{c|}{\textbf{Characterization}} & \multicolumn{1}{c|}{\textbf{Description from NIST VDO Ontology (NISTIR 8138)}~\cite{booth2016draft}} \\ \hline
Mitigation & \textbf{ASLR} & Some form of Address space layout randomization (ASLR) is in use. \\ \hline
Mitigation & \textbf{Multi-Factor Authentication} & Some form of Multi-Factor Authentication is required to access the product. \\ \hline
Mitigation & \textbf{Sandboxed} & The product is deployed within a sandbox \\ \hline
Mitigation & \textbf{HPKP} & HTTP Public Key Pinning (HPKP) is in use \\ \hline
Mitigation & \textbf{HSTS} & HTTP Strict Transport Security (HSTS) is in use \\ \hline
Mitigation & \textbf{Physical Security} & Some form of physical security is in place that would mitigate this vulnerability. \\ \hline
Impact Method & \textbf{Context Escape} & The Vulnerability allows an adversary to exploit a trust mechanism by breaking out of a sandbox and into another workspace. One and only one Context value shall be associated with Context Escape. The association denotes where a sandbox breakout originated. \\ \hline
Impact Method & \textbf{Trust Failure} & Exploitation of the Vulnerability takes advantage of an assumed trust relationship leading to unexpected impacts. Examples include failures of inherent trust, failure to verify a communicator, or the content being transmitted. \\ \hline
Impact Method & \textbf{Man-in-the-Middle} & This is usually accomplished by exploiting a trust mechanism and tricking both ends of the communication channel into believing that they are communicating with the intended party. \\ \hline
Logical Impact & \textbf{Write} & The Vulnerability allows an adversary to cause a breach in the integrity of the Context through unauthorized modification or addition of data. \\ \hline
Logical Impact & \textbf{Read} & The Vulnerability allows an adversary to cause a breach of confidentiality by gaining unauthorized access to data in the Context. \\ \hline
Logical Impact & \textbf{Service Interrupt} & The Vulnerability allows an adversary to cause an unauthorized loss of availability by temporarily or permanently disabling all or a portion of the Context \\ \hline
Logical Impact & \textbf{Indirect Disclosure} & The Vulnerability allows an adversary to learn information about the Context, but the knowledge gained is not from a direct read operation. Examples include but are not limited to discovering memory locations protected by ASLR, information from side-channel attacks, or information gained from traffic analysis \\ \hline
Logical Impact & \textbf{Privilege Escalation} & The Vulnerability allows an adversary to gain a level of privilege that was not intended. Unlike the other Logical Impact noun group values, Privilege Escalation is intended to represent that anything the Privilege Level acquired can do, can be done by the adversary. \\ \hline
Location & \textbf{Memory} & The Logical Impact is able to occur within memory \\ \hline
Location & \textbf{File System} & The Logical Impact is able to occur within the file system \\ \hline
Location & \textbf{Network Traffic} & The Logical Impact is able to occur within network traffic \\ \hline
Scope & \textbf{Limited} & There are restrictions to the associated impact \\ \hline
Scope & \textbf{Unlimited} & There are no restrictions to the associated impact \\ \hline
\end{tabular}
\label{tab:attributeDescriptions}
\end{table*}


==> threatsToValidity.tex <==
\section{Threats to Validity}
\label{sec:threats}
In this section we acknowledge potential threats to the validity of our findings and our mitigations, categorized by threat type ~\cite{wohlin2012experimentation}.

\subsection{Construct Validity}
Construct validity considers whether the correct metrics were used to evaluate an experiment. To evaluate how well our classifiers performed the given task, we used metrics (precision, recall, F-measure) and validation techniques (stratified 10-fold cross validation) widely used in machine learning and natural language processing. Further, to tune the hyper-parameters for each of the \numClassifiers{} classifiers, we performed extensive stratified 10-fold cross validation experiments with different configurations and selected the configuration for each that produced the best accuracy and F-measure. We provided the exact Weka schemes for each classifier in Table~\ref{tab:wekaSchemes} so the exact configurations could be reproduced. 

\subsection{Internal Validity}
Internal validity is concerned with mitigation of bias. We used a manual labelling process to create our dataset of vulnerability description-attribute mappings. This work required strong background knowledge of software security security concepts and a familiarity with the Vulnerability Description Ontology. The researcher who performed these tasks had the required background knowledge, and the labels were also reviewed by another experienced member of the research group to ensure consensus. To mitigate the risks associated with our imbalanced training data, we used \textit{stratified} 10-fold cross validation (CV). This is the default CV setting in the Weka tool used for these evaluations, and adjustments were made only to the classifiers hyper-parameters. Therefore, it is possible that not configuring options for the stratified CV introduced bias into the evaluation.

\subsection{External Validity}
External validity is a measure of how an approach can be \textit{generalized}. To make sure our approach was relevant to current standards of vulnerability management, this study mined CVE report descriptions from the online, publicly available National Vulnerability Database (NVD). This is the de-facto source of multi-vendor vulnerability report data in the United States. Therefore, this data is widely used, respected, and accessible. Further, by using only the textual descriptions, the approach is not limited to data with a specfic format.

Another concern is the generalization of the classifier's success. To make sure the technique was not limited to a certain category of characterization, we collected descriptions related to 19 characterizations from 5 of the 18 categories in the NIST Vulnerability Description Ontology. We also used the Ratio of Best Performance to determine which classifier performed the best for the most individual characterizations. Finally, the experiment and evaluation methodology was designed to ensure that the only step needed to add more characterizations is an extension to the labeled training set. 
